Detection Transformer with Stable Matching

This paper is concerned with the matching stability problem across different decoder layers in DEtection TRansformers (DETR). We point out that the unstable matching in DETR is caused by a multi-optimization path problem, which is highlighted by the one-to-one matching design in DETR. To address this problem, we show that the most important design is to use and only use positional metrics (like IOU) to supervise classification scores of positive examples. Under the principle, we propose two simple yet effective modifications by integrating positional metrics to DETR's classification loss and matching cost, named position-supervised loss and position-modulated cost. We verify our methods on several DETR variants. Our methods show consistent improvements over baselines. By integrating our methods with DINO, we achieve 50.4 and 51.5 AP on the COCO detection benchmark using ResNet-50 backbones under 12 epochs and 24 epochs training settings, achieving a new record under the same setting. We achieve 63.8 AP on COCO detection test-dev with a Swin-Large backbone. Our code will be made available at https://github.com/IDEA-Research/Stable-DINO.

==> images_tex/fusion_weight_distribution.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{resources/fusion_final.png}
    \vspace{-0.3cm}
    \caption{linear weight distributions during model training. The ``early'', ``mid'', and ``late'' are used for the 5000 steps, *** steps, and 90000 steps, respectively. \shilong{Not easy to explain.. wait for more results...}
    }
    \label{fig:fusion_distribution}
    \vspace{-0.4cm}
\end{figure}

==> images_tex/hero_figure.tex <==
\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Comparison of our methods and baselines.}
\label{fig:long}
\end{figure}
